Integrating Graceful Degradation and Recovery through Requirement-driven Adaptation

Cyber-physical systems (CPS) are subject to environmental uncertainties such as adverse operating conditions, malicious attacks, and hardware degradation. These uncertainties may lead to failures that put the system in a sub-optimal or unsafe state. Systems that are resilient to such uncertainties rely on two types of operations: (1) graceful degradation, to ensure that the system maintains an acceptable level of safety during unexpected environmental conditions and (2) recovery, to facilitate the resumption of normal system functions. Typically, mechanisms for degradation and recovery are developed independently from each other, and later integrated into a system, requiring the designer to develop an additional, ad-hoc logic for activating and coordinating between the two operations. In this paper, we propose a self-adaptation approach for improving system resiliency through automated triggering and coordination of graceful degradation and recovery. The key idea behind our approach is to treat degradation and recovery as requirement-driven adaptation tasks: Degradation can be thought of as temporarily weakening original (i.e., ideal) system requirements to be achieved by the system, and recovery as strengthening the weakened requirements when the environment returns within an expected operating boundary. Furthermore, by treating weakening and strengthening as dual operations, we argue that a single requirement-based adaptation method is sufficient to enable coordination between degradation and recovery. Given system requirements specified in signal temporal logic (STL), we propose a run-time adaptation framework that performs degradation and recovery in response to environmental changes. We describe a prototype implementation of our framework and demonstrate the feasibility of the proposed approach using a case study in unmanned underwater vehicles.

==> motivating-example-undersea.tex <==
\section{Motivating Example}
\label{section:motivating-example}

% \begin{figure}[h]

% \begin{center}
% \resizebox{\textwidth/2}{!}{
% \begin{tabular}{||c c c c||} 
%  \hline
%   & Sensor 1 & Sensor 2 & Sensor 3\\
%  [0.5ex] 
%  \hline\hline
%  Rates (Hz) & 5 & 4 & 4 \\
%  Energy Per Reading (J) & 3 & 2.8 & 2.1 \\
%  Energy Per 5s (J) & 75 & 56 & 42 \\
%  \hline
% \end{tabular}}
% \end{center}


% \caption{Configuration specs for each sensor for the AUV}
% \end{figure}

% \simon{talk about AUV (autonomous underwater vehicle), or UUV (unmanned underwater vehicle}
Consider an autonomous underwater vehicle (AUV) executing a water rescue mission in unmapped territory, inspired by the example presented in the UNDERSEA artifact \cite{undersea-case-study}. There are various onboard sensors that map the space surrounding the underwater vehicle to ensure its safety and detect signs of the mission target. It requires the AUV to \textbf{receive at least 20 readings every 5 seconds} ($R_1$) in order to safely explore the region without missing the target. In addition, the operation of these onboard sensors consumes energy that also supports the movement and maneuvering of the AUV. To prevent disruption to the mission objectives and ensure the timeliness of the mission, we mandate that the \textbf{energy consumption of all sensors should not exceed 50 J every 5 seconds} ($R_2$). 

Suppose there is a scenario where one or more sensors degrade or fail due to environmental factors like sensor attack or hardware degradation, resulting in the system being unable to comply with the safety requirement, resulting in the system failing to plan a course of action that allows the vehicle to continue operating in a desired state. If the vehicle continues its movement without addressing these violations, it risks missing the target, or even running into underwater obstacles, which can cause more severe failure or damages. 

% In some cases, the system can be reconfigured to meet these requirements again. For example, this may entail replacing the primary sensor with a less efficient sensor. However, in the case where no possible configuration is possible to meet the requirement given the system capability. \simon{to be changed?}

% talk about the restart (enter recovery mode, inability to progress), checkpointing (deviate from actual system stats), setpoint (reconfigure the system according to the setpoint), 

\paragraph{Existing Methods}
% system restart
One of the conceptually simple approaches to recovery from this failure is through a full system restart \cite{abad16} \cite{jagtap20}, where the sensors are temporarily taken offline to allow diagnosis and repair of the degraded or failed sensors. However, this approach is not desirable as it risks disrupting the system's operation, in this case, means stopping the mission of the vehicles due to the lack of situational awareness because of the reduced sensing capability, which can result in the loss of mission during the critical phase. 

% checkpointing
Checkpointing is another recovery approach that leverages historical system state information (like the location of the vehicle, water current, speed, etc.) and an environmental model, to approximate future system states to compensate for the effect of sensor failure. However, the limitation of this approach is that it is not suitable for persistent failures, in which case the approximated future states can deviate significantly from reality, resulting in safety violations.

% setpoint
Another recovery approach that leverages a concept in control theory is called setpoint, which is a desired value for a system parameter. For example, to recover from the sensor failures, we can set the desired value for the sensor throughput (per 5 seconds) to 20 (\textit{SP1}), and the energy consumption (per 5 seconds) to 50 (\textit{SP2}). A controller can be designed based on these setpoints that capture the system requirements and synthesize control actions that allow the system to maintain these setpoints throughout its operation. However, the fixed setpoints may result in a brittle system when the setpoints are impossible to satisfy. For example, in the case that sensor 3 fails, no other configuration of the system can reach the setpoint in the next control loop given the failure.

% The majority of the work in the existing self-adaptive system (SAS) research focuses on utilizing adaption tactics to accomplish the defined system goals with the ultimate objective of maximizing the system utility defined by the user based on some quality of service (QoS) attributes. For example, the user can provide a utility function $U = w_1 E + w_2 R$ where $E$ and $R$ indicate the energy consumption and number of readings throughout the span of 5 seconds ($w_1$ and $w_2$ are arbitrary weights defined by the user), and the system will choose tactics that maximize the utilities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Disadvantage of utility function %
% lack of traceability %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% While the utility function provides a powerful way to define the goodness of the system with respect to some desired properties, there are a few challenges with the utility function approach: (1) The expressive of the utility function is limited. For example, the utility function itself doesn't express anything related to the temporal aspects of the system execution (i.e. a property should hold within a certain time period) (2) the metric itself does not provide insights into whether the system guarantees certain properties. For example, suppose the system ended up choosing a tactic that selects sensor 1, while its rate configuration satisfies the requirement, its energy consumption exceeds that of required by the system. But this is not reflected in the utility function in any way. There seems to be a lack of a mechanism to relate the utility score back to the satisfaction of individual requirements. Therefore, it's a common practice to optimize for the utility function given some hard constraints are satisfied first\simon{cite UNDERSEA paper}.

% However, this leads to another set of problems. The desired requirement specified during design time that serves a setpoint during runtime can be overly restrictive to the point that the Planner (P) of the MAPE-K self-adaptation loop cannot generate any valid plans according to this setpoint given the environmental disruption. In our example, this will happen when sensor 3 fails, resulting in the system being unable to meet $R_2$, leading to the system being unable to generate any adaptation tactics to fulfill $R_2$, which will eventually trigger cascading failures resulting in mission failure and loss of the vehicle.

% talk about the degradation step and recovery step 
\paragraph{Proposed Method}: Our approach consists of two steps. First, it attempts to compensate for the failure by degrading the system functionality through relaxing the desired requirement that the system is required to satisfy initially, thus making it easier for the planner to synthesize plans based on the weakened requirement. Secondly, from that point on, based on the system capability at any arbitrary time, the  system continuously seeks opportunities to improve the system by incrementally strengthen the weakened requirement, to the best possible requirement achievable, and in the best-case scenario, to the original desired requirement.

For example, recall we have the desired requirement of the system as follows:

$R_1$: \textit{The sensors should receive at least 20 readings within 5 seconds.}\

$R_2$: \textit{The energy consumption of all the sensors should not exceed 50 J within 5 seconds.}

Imagine a scenario where both sensor 3 and sensor 2 (the more efficient sensors among the set of sensors) fails, in which case it violates the original requirement $R_1 \land R_2$, as sensor 1 violates the energy consumption requirement $R_2$ in the case that it is turned on, and the system violates the throughput requirement $R1$ when it is turned off. However, given the remaining system capability (i.e. sensor 1 remains operational), the system may choose to degrade the energy consumption requirements $R_2$ to $R_2'$ below:

$R_2'$: \textit{The energy consumption of all the sensors should not exceed 75 J within 5 seconds.}

%Note that we are making the assumption that user defines a minimal requirement, that is, a requirement below which the system ceases to be operational (for example, in our case, this may entail engine is required to shut down to preserve the system's energy), all the weakened requirement should be stronger than the minimal requirement. 
With the new weakened requirement $R_1 \land R_2'$, the recovery planner, may emit actions like temporarily bring sensor 1 online, ensuring the throughput requirement by temporarily sacrificing the energy consumption requirements. Furthermore, the weakening of the energy consumption requirement may trigger adaptations in other components of the system, for example, by reducing the speed of the vehicles to compensate for the increased energy consumption of the sensors, to further stabilize the system.
% should we talk about reducing the speed as well?

The recovery step involves gradually strengthen the requirements given the current operating conditions. Suppose sensor 2 resumes operational at certain point, given the monitor reliably detects the "sensor 2 repaired" event, we are first strengthen the requirement from $R_2'$ to $R_2''$ like follows:

$R_2''$: \textit{The energy consumption of all the sensors should not exceed 56 J within 5 seconds.}

In which case, the planner may synthesize actions like "turn on sensor 2, turn off sensor 1" to comply with the updated requirement. Similarly, in the case where sensor 3 is back online, the requirement resumes to the original requirement $R_2$. In the case where there's persistent failure for sensor 3, the reference requirement remains at $R_2''$ for the remaining of the mission.

\paragraph{Challenges}
\simon{(1) finding the range of weakened requirements (minimal requirement) {2} determine the amount of degradation or recovery based on environmental model and system capability}
% \simon{Talk about self-adaptive system, and the notion of tactics}
% maximizing the utility

% \simon{preventing from tracing t}
% \simon{sensor 3 and sensor 2 fails, sensor 1 is enabled}
% % \simon{disadvantage}



% \newpage;
% \textbf{Case study 1}

% % https://www-users.york.ac.uk/~sg778/UNDERSEA/
% The UUV is equipped with various sensors of varying levels of qualities)

% \textbf{R1 (throughput)}: The UUV should take at least 20 readings of sufficient accuracy within the next 10 seconds.

% \textbf{R2 (resource usage)}: The energy consumption of the sensors should not exceed 120 Joules within the next 10 seconds.

% Suppose due to environmental uncertainties, the sensors may be subject to failures, resulting in these requirement being violated. The goal is trying to plan for the 

% These requirements can be formalized to the following STL requirements
